FreqKV: Key-Value Compression in Frequency Domain for Context Window Extension

Existing key-value (KV) cache compression methods for large language models (LLMs) often rely on token eviction, which risks losing critical local information in both long prefilling and decoding scenarios. When extrapolating beyond the pretrained context length, their performance degrades sharply on long-context benchmarks. Motivated by the observation in the frequency domain that the context information is concentrated in the low-frequency components, we propose FreqKV, a parameter-free and architecture-agnostic approach. It iteratively compresses the increasing KV cache in the frequency domain, allowing models to process lengthy contexts efficiently. With minimal training at 8K length, FreqKV extends the context window of LLaMA-2-7B up to 256K tokens while maintaining stable perplexity. Extensive experiments across prefilling and decoding demonstrate that FreqKV enables robust context window extension and consistently outperforms existing KV cache compression methods on LLaMA-2 and LLaMA-3, highlighting its effectiveness for both understanding and generation in long contexts.

==> figtex/compression.tex <==
\begin{wrapfigure}{r}{0.27\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/compression.pdf}
    \caption{The illustration of the frequency-domain compression.}
    \label{fig:compression}
\end{wrapfigure}

==> figtex/cost.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/time.pdf} 
    \caption{Decoding time with the full cache and FreqKV on the increasing sequence length.}
    \label{fig:decoding-time} 
\end{figure}


==> figtex/minigape.tex <==
\begin{figure*}[!ht]
    \centering
    % 第一张图片
    \begin{minipage}{0.42\textwidth}
        \centering
        \captionof{table}{Performance of different KV compression methods on LongGenBench.}
        \label{tab:LongGenBench}
        \begin{tabular}{lcc}
        \toprule
        \bf Method & \bf GSM8K & \bf MMLU \\
        \midrule
        LLaMA-3 & 42.8 & 23.8 \\
        \, +D2O & 8.0 & 24.8 \\
        \, +FastKV & 48.5 & 25.4 \\
        \, +SnapKV & 49.6 & 25.8 \\
        \, +PyramidKV & 49.6 & 26.2 \\
        \bf \, +FreqKV & \bf 54.2 & \bf 31.2 \\
        \bottomrule
        \end{tabular}
        % \label{fig:training-cost} 
    \end{minipage}
    \hspace{0.01\textwidth}  % 两张图片之间的间距
    \begin{minipage}{0.55\textwidth}
    \hspace{-0.5em}
    \subfloat[Dropping.]{
        \includegraphics[width=0.491\linewidth]{figures/needle-llama2-drop.pdf}}
    \hspace{-0.5em}
    \subfloat[FreqKV.]{
        \includegraphics[width=0.514\linewidth]{figures/needle-llama2-freqkv.pdf}}
    \caption{Comparison of FreqKV and its variant Dropping on LLaMA-2-chat-7B.}
    \label{fig:needle-llama2-drop} 
    \end{minipage}
\end{figure*}


==> figtex/needle-llama2.tex <==
\begin{figure} [!ht]
	\centering
	\subfloat[\label{fig:needle-llama2-freqkv}The Needle-in-a-Haystack results of FreqKV on LLaMA-2-chat-7b. The average accuracy is 84.2\%.]{
		\includegraphics[width=\linewidth]{figures/needle-llama2-freqkv.pdf}}
        \\
        \subfloat[\label{fig:needle-llama2-snapkv}The Needle-in-a-Haystack results of SnapKV on LLaMA-2-chat-7b. The average accuracy is 46.7\%.]{
		\includegraphics[width=\linewidth]{figures/needle-llama2-snapkv.pdf}}
        % \hspace{-0.5cm}
	\caption{The Needle-in-a-Haystack results of LLaMA-2-chat-7b, with the x-axis representing the document length (“haystack”) ranging from 1K to 8K tokens, and the y-axis showing the position of the “needle” (a short sentence) within the document.
 }
	\label{fig:needle-llama2} 
\end{figure}

==> figtex/needle-llama3.tex <==
\begin{figure} [!ht]
	\centering
	\subfloat[\label{fig:needle-llama3-freqkv}The Needle-in-a-Haystack results of FreqKV on LLaMA-3-instruct-8b. The average accuracy is 90.7\%.]{
		\includegraphics[width=\linewidth]{figures/needle-llama3-freqkv.pdf}}
        \\
        \subfloat[\label{fig:needle-llama3-snapkv}The Needle-in-a-Haystack results of SnapKV on LLaMA-3-instruct-8b. The average accuracy is 52.3\%.]{
		\includegraphics[width=\linewidth]{figures/needle-llama3-snapkv.pdf}}
        % \hspace{-0.5cm}
	\caption{The Needle-in-a-Haystack results of LLaMA-3-instruct-8b, with the x-axis representing the document length (“haystack”) ranging from 1K to 16K tokens.
 }
	\label{fig:needle-llama3} 
\end{figure}

==> figtex/niah-llama2.tex <==
\begin{figure*} [!t]
	\centering
    	\subfloat[\label{fig:niah-llama2-freqkv}The Needle-in-a-Haystack results of FreqKV. The average accuracy is 86.8\%.]{
            \hspace{-0.3cm}
		\includegraphics[scale=0.163]{figures/freqkv2llama_2_7b.pdf}}
        \\
        \subfloat[\label{fig:niah-llama2-localkv}The Needle-in-a-Haystack results of ``Local Attention". The average accuracy is 75.5\%.]{
            \hspace{-0.3cm}
		\includegraphics[scale=0.163]{figures/localkvllama_2_7b.pdf}}
        \\
        \subfloat[\label{fig:niah-llama2-snapkv}The Needle-in-a-Haystack results for SnapKV show an average accuracy of 49.6\%, which drops sharply when the context length exceeds LLaMA2's 4k token window.]{
            \hspace{-0.3cm}
		\includegraphics[scale=0.163]{figures/snapkvllama_2_7b.pdf}}
        % \hspace{-0.4cm}
	\caption{The Needle-in-a-Haystack resultson  LLaMA-2-Chat-7B, with the x-axis representing the document length (“haystack”) ranging from 1K to 8K tokens, and the y-axis showing the position of the “needle” (a short sentence) within the document.}
	\label{fig:niah-llama2} 
\end{figure*}

==> figtex/retaining-ratio.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\linewidth]
    {figures/retaining-ratio.pdf}
    \caption{Perplexity evaluation on the validation set of PG-19 with different retaining ratios. The training context length is 8192.}
    \label{fig:retaining-ratio}
\end{figure}
